End-to-End Optimization of Scene Layout

We propose an end-to-end variational generative model for scene layout synthesis conditioned on scene graphs. Unlike unconditional scene layout generation, we use scene graphs as an abstract but general representation to guide the synthesis of diverse scene layouts that satisfy relationships included in the scene graph. This gives rise to more flexible control over the synthesis process, allowing various forms of inputs such as scene layouts extracted from sentences or inferred from a single color image. Using our conditional layout synthesizer, we can generate various layouts that share the same structure of the input example. In addition to this conditional generation design, we also integrate a differentiable rendering module that enables layout refinement using only 2D projections of the scene. Given a depth and a semantics map, the differentiable rendering module enables optimizing over the synthesized layout to fit the given input in an analysis-by-synthesis fashion. Experiments suggest that our model achieves higher accuracy and diversity in conditional scene synthesis and allows exemplar-based scene generation from various input forms.

==> 04_model.tex <==
\section{Image Formation Model}
Our main idea is to bring mature graphics rendering engines into the task of conditional image synthesis, but augmenting it with modern neural networks. Such a combination unifies the strengths of both worlds. Graphics engines build upon the classic rendering equation~\cite{kajiya1986rendering} and produce realistic images; they however require pre-specified scene layout and object texture and lighting as input. The distribution of real-life scene layout, texture, and lighting is highly complex; therefore, we propose to use deep generative models to approximate these distributions.

Think about how an image is formed. At the high level, the layout of the scene suggests ‘what is
 where’, as well as the relations between the objects. At the middle level, each object in the image has its distinct shape and pose. At the low level, object patches have complex texture and the entire scene can have lighting. Thus, our specific model design can be summarized as
\begin{center} Image = \textit{Layout + Shape + Texture + Lighting} \end{center}
The disentangled representation allows us to modify each aspect of the image synthesis process independently. Utilizing this disentangled representation, we demonstrate 3D layout refinement with supervision only 2.5D sketches.


==> plots/process.tex <==
\begin{figure*}[t]
\vspace{-0.1in}
 \begin{center}
  \includegraphics[width=0.8\textwidth]{plots/fig_process.pdf}
  \captionsetup{width=.8\linewidth}
  \caption{Our model for conditional image synthesis. We use a conditional variational autoencoder (cVAE) to generate scene layouts from scene graphs, followed by object retrieval and then a conditional GAN to generate texture. The image is rendered by a graphics engine}
  \label{fig:process}
  \end{center}
  \vspace{-0.3in}
\end{figure*}

==> plots/relationships.tex <==
\begin{table}[]
\begin{tabular}{l|l}
Relationships   & Attributes \\ \hline
left of         & None       \\
right of        & Tall       \\
behind          & Short      \\
in front of     & Large      \\
inside          & Small      \\
surrounding     &            \\
left touching   &            \\
right touching  &            \\
top touching    &            \\
bottom touching &            \\
on              &           
\end{tabular}
\end{table}

==> plots/relationships_hori.tex <==
\begin{table}[]
\begin{tabular}{l|lllllllllll}
Relationships & left of & right of & behind & in front of & inside & surrounding & left touching & right touching & top touching & bottom touching & on \\ \hline
Attributes    & None    & Tall     & Short  & Large       & Small  &             &               &                &              &                 &   
\end{tabular}
\end{table}
